Vibrational and stochastic resonances in two coupled overdamped anharmonic oscillators

We study the overdamped version of two coupled anharmonic oscillators under the influence of both low- and high-frequency forces respectively and a Gaussian noise term added to one of the two state variables of the system. The dynamics of the system is first studied in the presence of both forces separately without noise. In the presence of only one of the forces, no resonance behaviour is observed, however, hysteresis happens there. Then the influence of the high-frequency force in the presence of a low-frequency, i.e. biharmonic forcing, is studied. Vibrational resonance is found to occur when the amplitude of the high-frequency force is varied. The resonance curve resembles a stochastic resonance-like curve. It is maximum at the value of $g$ at which the orbit lies in one well during one half of the drive cycle of the low-frequency force and in the other for the remaining half cycle. Vibrational resonance is characterized using the response amplitude and mean residence time. We show the occurrence of stochastic resonance behaviour in the overdamped system by replacing the high-frequency force by Gaussian noise. Similarities and differences between both types of resonance are presented.

==> wideabs <==
  You can actually get a first page that looks something like the first
page of Phys. Rev. (with abstract across the page), IF you are using
version 3.1 of REVTeX. Here is the general format:

\wideabs{
\title{ . . . }
   .
   .
   .
\pacs{ . . . }
}

That is, just insert the command \wideabs the title, and put the
ending curly brace after the pacs.

  Note that these lines should never appear in a file destined for the APS.
Note also that this is a quick hack and may have unknown drawbacks, along
with these known ones:

  (1) Byline footnotes (any footnotes or \thanks between the inserted lines)
      will probably just disappear.
  (2) No catcode changes can be effected between the inserted lines;
      mainly this means no verbatim and \verb, but may have other
      consequences.
It was intended to produce a style that had the abstract printed on the
width of the page, but there were always problems with the implementation and
so it was withdrawn near the release date. It may be possible to solve this
problem in the future.





